Level-Set Topology Optimization for Ductile and Brittle Fracture Resistance Using the Phase-Field Method

This work presents a rigorous mathematical formulation for topology optimization of a macrostructure undergoing ductile failure. The prediction of ductile solid materials which exhibit dominant plastic deformation is an intriguingly challenging task and plays an extremely important role in various engineering applications. Here, we rely on the phase-field approach to fracture which is a widely adopted framework for modeling and computing the fracture failure phenomena in solids. The first objective is to optimize the topology of the structure in order to minimize its mass, while accounting for structural damage. To do so, the topological phase transition function (between solid and void phases) is introduced, thus resulting in an extension of all the governing equations. Our second objective is to additionally enhance the fracture resistance of the structure. Accordingly, two different formulations are proposed. One requires only the residual force vector of the deformation field as a constraint, while in the second formulation, the residual force vector of the deformation and phase-field fracture simultaneously have been imposed. An incremental minimization principles for a class of gradient-type dissipative materials are used to derive the governing equations. Here, the level-set-based topology optimization is employed to seek an optimal layout with smooth and clear boundaries. Sensitivities are derived using the analytical gradient-based adjoint method to update the level-set surface for both formulations. Here, the evolution of the level-set surface is realized by the reaction-diffusion equation to maximize the strain energy of the structure while a certain volume of design domain is prescribed. Several three-dimensional numerical examples are presented to substantiate our algorithmic developments.

==> MCFEM.tex <==
 


%%=======================================================================
\sectpa[Section3]{The stochastic phase-field fracture}
We consider a probability space $(\Omega, \mathbb{A},
\mathbb{P})$, where $\Omega$ indicates the set of elementary events (
the sample space), $\mathbb{A}$ is the $\sigma$-algebra of all possible
events, and $\mathbb{P}\colon \mathbb{A} \to [0,1]$ is a probability
measure. A real-valued random variable $\xi:\Omega\rightarrow\mathbb{R}$ is a set of possible events ($\Omega$), mapping the probability space to the real values. Here, we assumed that the random variable is Gaussian (has normal ditsribution), i.e. they have the following probability density function 
\begin{align}
	\mathbb{P}(\omega)=\frac{1}{\sqrt{2\pi\sigma^2}} \exp\frac{(\omega-\mu)^2}{2\sigma^2}.
\end{align}
For the Gaussian random variables, the probability density function considers two components, namely the mean value ($\mu$) and the variance ($\sigma$). Exceptionally, once we have $\mu=0$ and $\sigma=1$, we call the random variable, standard normal. Here, for a more realistic case, we use uniformly distributed random variables.



Now, we define an inner product $	\langle \xi,\zeta\rangle_{\mathcal{A}}=\mathbb{E}\left[ \xi\,\zeta\right]$ and the following Lebesgue space of the random variables with the finite variance
\begin{align}
	\mathcal{A}:=L_2(\Omega,\mathbb{R})=\{\xi:\Omega\rightarrow\mathbb{R}:~~\|\xi\|_{\mathcal{A}}^2:=	\langle \xi,\xi\rangle_{\mathcal{A}}=\mathbb{E}[\xi^2]<\infty\}.
\end{align}
Using the above-mentioned definition, we define the the covariance operator given by $\mathcal{COV}(\xi,\zeta):=\mathbb{E}\left[\left( \xi-\mathbb{E}[\xi]\right)\left( \zeta-\mathbb{E}[\zeta]\right)  \right]= \langle \xi-\mathbb{E}[\xi],\zeta-\mathbb{E}[\zeta] \rangle_{\mathcal{A}}$. Obviously, the variance function can be defined $\mathbb{V}(\zeta)=\mathcal{COV}(\zeta,\zeta)$. We can set the uncorrelated random variables when we have $\mathcal{COV}(\xi,\zeta)$=0.
A random variable $\xi(\boldsymbol{x},\omega):\Omega\times X\rightarrow \mathbb{R}$ is related to the spatial variable $\boldsymbol{x}\in X$ and the random variable $\xi\in\Omega$. Considering the fixed random variable $\omega\in\Omega$, $\xi(\omega,\cdot)$ indicates the deterministic cases, which is one observation in the phase-field problem (ductile/brittle).   
 
We denote a quantity of interest (QoI) as a function of $(\boldsymbol{u}, \varphi, \alpha) \in X\times X\times X$ (\todo{Amir: write the solution spaces}) shown by $\Delta (\boldsymbol{u}, \varphi, \alpha)$. Considering the randomness, we have the effect of the random variable on the solution, and then we have $\Delta (\boldsymbol{u} (\omega), \varphi (\omega), \alpha(\omega))$. Therefore, we normally compute the expectation of QoI denoting $\boldsymbol{\Delta}=\mathbb{E}\left[\Delta (\boldsymbol{u} (\omega), \varphi (\omega), \alpha(\omega))\right]$.
 
 
 
  In a Monte Carlo finite-element (FE) method several evaluations
 are combined   to obtain an approximation of the solution of
 the model equation or equations.
 Considering the Bochner space $L^2(\Omega;X)$ for the mappings $\mathcal{Y}\colon \Omega \to X$, we can define
 \begin{align}\label{bochner norm}
 	\| \mathcal{Y} \|_{L^2(\Omega;X)} :=\Big( \int_\Omega \| \mathcal{Y}(\cdot,\omega) \|_X^2 \,\P(\omega)
 	\Big)^{1/2}
 	= \E\Big[\| \mathcal{Y}(\cdot,\omega) \|_X^2 \Big]^{1/2}.
 \end{align}
Here, the variance function is given by $\mathbb{V} ( \mathcal{Y}) = \|\E[ \mathcal{Y}]- \mathcal{Y}\|_{L^2(\Omega;D)}^2$
 We consider the quantity of interest $\mathcal{X}$,  the standard MC estimator $\EMC$ for
 $\mathbb{E}[\mathcal{X}]$ is the sample mean
 \begin{equation}\label{MC-estimator}
 	\EMC[\mathcal{X}]
 	:= \frac{1}{M} \sum_{i=1}^{M} \mathcal{X}^{(i)},
 \end{equation}
 where $ \mathcal{X}^{(i)}$ is the $i$-th sample (independent random variable) of $ \mathcal{X}$. $\mathcal{X}$ is the function of ...............
 
 A perturbed (material) parameter can be defined using the perturbation value $\eta$ as
 \begin{align}
 	\chi=\bar{\chi}+\eta \tilde{\theta},
 \end{align}
where $\tilde{\theta}$ is a uniformly distributed random variable in [-1,\,1].

==> NN_lit.tex <==

@article{noii2019phase,
	title={A phase-field description for pressurized and non-isothermal propagating fractures},
	author={Noii, Nima and Wick, Thomas},
	journal={Computer Methods in Applied Mechanics and Engineering},
	volume={351},
	pages={860--890},
	year={2019},
	publisher={Elsevier}
}

@article{noii2020adaptive,
	title={An adaptive global--local approach for phase-field modeling of anisotropic brittle fracture},
	author={Noii, Nima and Aldakheel, Fadi and Wick, Thomas and Wriggers, Peter},
	journal={Computer Methods in Applied Mechanics and Engineering},
	volume={361},
	pages={112744},
	year={2020},
	publisher={Elsevier}
}

@article{noii2021bayesian,
	title={Bayesian inversion for anisotropic hydraulic phase-field fracture},
	author={Noii, Nima and Khodadadian, Amirreza and Wick, Thomas},
	journal={Computer Methods in Applied Mechanics and Engineering},
	volume={386},
	pages={114118},
	year={2021},
	publisher={Elsevier}
}

@article{aldakheel2021multilevel,
	title={Multilevel global--local techniques for adaptive ductile phase-field fracture},
	author={Aldakheel, Fadi and Noii, Nima and Wick, Thomas and Allix, Olivier and Wriggers, Peter},
	journal={Computer Methods in Applied Mechanics and Engineering},
	volume={387},
	pages={114175},
	year={2021},
	publisher={Elsevier}
}

@article{noii2021quasi,
	title={A quasi-monolithic phase-field description for orthotropic anisotropic fracture with adaptive mesh refinement and primal--dual active set method},
	author={Noii, Nima and Fan, Meng and Wick, Thomas and Jin, Yan},
	journal={Engineering Fracture Mechanics},
	volume={258},
	pages={108060},
	year={2021},
	publisher={Elsevier}
}

@article{noii2022bayesian,
	title={Bayesian Inversion with Open-Source Codes for Various One-Dimensional Model Problems in Computational Mechanics},
	author={Noii, Nima and Khodadadian, Amirreza and Ulloa, Jacinto and Aldakheel, Fadi and Wick, Thomas and Fran{\c{c}}ois, Stijn and Wriggers, Peter},
	journal={Archives of Computational Methods in Engineering},
	pages={1--34},
	year={2022},
	publisher={Springer}
}

@article{ulloa2022variational,
	title={Variational modeling of hydromechanical fracture in saturated porous media: A micromechanics-based phase-field approach},
	author={Ulloa, Jacinto and Noii, Nima and Alessi, Roberto and Aldakheel, Fadi and Degrande, Geert and Fran{\c{c}}ois, Stijn},
	journal={Computer Methods in Applied Mechanics and Engineering},
	volume={396},
	pages={115084},
	year={2022},
	publisher={Elsevier}
}

@article{noii2022probabilistic,
	title={Probabilistic failure mechanisms via Monte Carlo simulations of complex microstructures},
	author={Noii, Nima and Khodadadian, Amirreza and Aldakheel, Fadi},
	journal={Computer Methods in Applied Mechanics and Engineering},
	volume={399},
	pages={115358},
	year={2022},
	publisher={Elsevier}
}

@article{noii2022bayesian,
	title={Bayesian Inversion Using Global-Local Forward Models Applied to Fracture Propagation in Porous Media},
	author={Noii, Nima and Khodadadian, Amirreza and Wick, Thomas},
	journal={International Journal for Multiscale Computational Engineering},
	volume={20},
	number={3},
	year={2022},
	publisher={Begel House Inc.}
}

@article{liu2022phase,
	title={Phase field modeling of brittle fracture in large-deformation solid shells with the efficient quasi-Newton solution and global--local approach},
	author={Liu, Z and Reinoso, J and Paggi, M},
	journal={Computer Methods in Applied Mechanics and Engineering},
	volume={399},
	pages={115410},
	year={2022},
	publisher={Elsevier}
}

==> doc1.tex <==


the total energy functional (higher
stiffer material response)

A critical and popular issue in density-based topology optimization on a 
fixed mesh of finite elements is the mesh dependency phenomenon, which 
precautions must be taken to avoid it. As the name suggests, the mesh 
dependency phenomenon refers to obtaining qualitatively different 
solutions for different mesh sizes or number of discretization points. 
Through the results, it is concluded that the proposed method has mesh dependency.



The key requirement for realizing this

Additionally, in the present study, the displacement-control adjoint sensitivity for topology optimization is used. 

In order to derive the gradient-based fully coupled adjoint-based sensitivity analysis, derivatives of the objective and constraint functions with respect to the design variables need to be provided to evolve the structural topology. 

None of the aforementioned continuum buckling works have included the effects of elasto-
plastic material response. This may be due to a number of factors, the most important of
which being the very large computational burden associated with not only a nonlinear forward analysis in which large deformation kinematics may be used and arc-length methods may be required, but also the sensitivity analysis associated with buckling load factors.

models may be used


Level-set topology optimization of fracture-Resistance of macro structure undergoing ductile failure


This is accomplished by introducing

Due to the softening behavior caused by material degradation arising from crack growth and fracture, which leads to decreased material integrity drastically, the fracture is one of the most common failure modes in structures, which reduces significantly the load-bearing capacity. This becomes even more important when known that the optimization process often leads to slender and weak members which are very sensitive with respect to nonlinear phenomena such as the fracture. 


++++++++++++++++++++

by HASAN:

=============


to this setting would
pave the way for a wide adoption of phase-field modeling of fracture, already well
established in the research community, within legacy codes for industrial applications. 


With regard to various nonlinearity sources, the reaction-diffusion based level set approach proposed by \cite{Jahan_IGA_LSM_RDE2, JAHANGIRY2022103358}.

With the aim of more realistic designs, many efforts have been conducted to develop topology optimization into nonlinear structural designs considering various nonlinearity sources. The gradient-based topology optimization of materially nonlinear structures has been conducted by several researchers \cite{schwarz2001topology, yoon2007topology, huang2007topology, huang2008topology, bogomolny2012conceptual, xia2017evolutionary, maury2018elasto, zhao2019material, zhao2020topology}.
+++++++++++++++++++

\TODO{MESH SENSITIVITY}

=============================

In the following, we describe in more detail our main goals.
First, we focus on the development of Global-Local
formulation for ductile fracture. {Specifically}, the continuum phase-field approach to ductile fracture
is employed. 


=============================
The second objective is to introduce  a predictor-corrector
adaptivity within the Global-Local concept to reduce the computational time. 


{The} key requirement for realizing {this} ....


******************************************************************************************
Abstract:

A critical and popular issue in density-based topology optimization on a 
fixed mesh of finite elements is the mesh dependency phenomenon, which 
precautions must be taken to avoid it. As the name suggests, the mesh 
dependency phenomenon refers to obtaining qualitatively different 
solutions for different mesh sizes or number of discretization points. 
Through the results, it is concluded that the proposed method has mesh dependency.

******************************************************************************************

Conclusion:

Intending to evaluate the mesh sensitivity in the proposed numerical method, the 
results were obtained in Three various types of mesh sizes. Finer meshes lead to 
a qualitative distribution of materials with higher numbers of holes, which is 
capable to provide more optimal results than coarser meshes. However, finer meshes 
may lead to more complex structures that are difficult to manufacture.The obtained 
results show that the proposed method has mesh dependency. 



==> numerical.tex <==


 


%=======================================================================
\sectpa[Section4]{Numerical examples}
%=======================================================================



\setcounter{table}{0}
\begin{table}[!ht]
	\caption{Material parameters used in the numerical experiments. The fixed values in all examples are mentioned. Other parameters are inferred with Bayesian inversion.}	\vspace{1mm}
	\centering
	\begin{tabular}{cllcccccc}
		Parameter & Name                  & Unit       & Value     \\[2mm]\hline 
		$\mu$        & shear modulus    &     $\mathrm{MPa}$ &$\mathrm{BI}$ \\[2mm]
		$K$      & bulk modulus    &   $\mathrm{MPa}$     &$\mathrm{BI}$       
		\\[2mm]
		$H$        & hardening modulus         & $\mathrm{MPa}$ &$\mathrm{BI}$\\[2mm]
		$\sigma_Y$        & yield stress      & $\mathrm{MPa}$&$\mathrm{BI}$ \\[2mm]
		$\psi_c$     & specific fracture energy    & $\mathrm{MPa}$ &$\mathrm{BI}$\\[2mm]
		$G_c$     & Griffith's energy release rate     & $\mathrm{MPa}$ &$\mathrm{BI}$\\[2mm]
		$\zeta$    &driving scaling factor&--&$\mathrm{BI}$\\[2mm]
		$\eta_f$    & crack viscosity       & $\mathrm{N/m^{2}s}$&$10^{-9}$\\[2mm] 
		$\eta_p$    & plasticity viscosity       & $\mathrm{N/m^{2}s}$&$10^{-9}$\\[2mm] 
		$\kappa$    & stabilization parameter   & -- & $10^{-8}$& & \\[2mm]
		$l_d$    & fracture length-scale  &  $\mathrm{mm}$  & $10^{-8}$ & \\[2mm]
		$l_{\Phi}$    & topology length-scale     &$\mathrm{mm}$& $10^{-4}$ \\[2mm]
		$r_{min}$    & filtering radius     &$\mathrm{mm}$& $10^{-4}$ \\[2mm]
		$v_{max}$    & volume fraction     &--& $40\%$ \\[2mm]
		$\tau_d$    & volume fraction     &--& $1\times10^{-4}$ \\[2mm]
		$\tau_{\Phi}$    & volume fraction     &--& $0.1$ \\[2mm]
		$c$    & mapping power between inclusion/matrix     &--& $2$ \\[2mm]
		\hline
		\label{material-parameters}
	\end{tabular}
\end{table}


$r_{min}=3l_d$
 
 $\tau=10^{-4}$
 
 $dt=0.1$


==> sec3.tex <==
%=======================================================================
\sectpa[Section3]{Topology Optimization for Fracturing Material}
%=======================================================================

%
In a general, a mathematical formulation of topological optimization problem for the given functional $\BfrakL(\BfrakU)$  subject to the equality/inequality constrains reads:
% \BfrakL
%
\begin{equation}\label{compat_argmin}
		\Phi = 
		\substackrel{\Phi \in \bf{V} }{\mbox{argmin}}\,
		\Big\{[\;\BfrakL(\BfrakU)] \quad |\quad 
	\BfrakR(\BfrakU)=0 \AND \BfrakG(\BfrakU)\leq G^\star \Big\}
\end{equation}
%
for unknown parameters $\Phi$ with
%
\begin{equation} 
	\begin{aligned}
		&\BfrakL(\BfrakU)
		=\int_{\calB}{\widehat{F}}(\Bu,d,\Phi)  \mathrm{d}{\bm{x}} 
		\WITH \widehat{F}(\Bu,d,\Phi)=F(\Bu,d,\Phi)\text{H}^{c_1}(\Phi),\\
		&\BfrakR(\BfrakU)
		=\int_{\calB}{\widehat{R}}(\Bu,d,\Phi)  \mathrm{d}{\bm{x}} 
		\WITH \widehat{R}(\Bu,d,\Phi)=R(\Bu,d,\Phi)\text{H}^{c_2}(\Phi),\\
		&\BfrakG(\BfrakU)
		=\int_{\calB}{\widehat{G}}(\Bu,d,\Phi)  \mathrm{d}{\bm{x}} 
		\WITH \widehat{G}(\Bu,d,\Phi)=G(\Bu,d,\Phi)\text{H}^{c_3}(\Phi).
	\end{aligned}
\end{equation}		
%
Here, $ \BfrakL(\BfrakU)$ is a functional with its density function $ \widehat{F} $ for a global primary fields $ \BfrakU$ within the structural design domain $ \calB $. The minimization problem is subjected to equality  constraint functional as $\BfrakR(\BfrakU)$ with its density $ \widehat{R} $, along with  inequality  constraint functional denoted as $\BfrakG(\BfrakU)$ with its density $  \widehat{G}$. To  resolve \req{compat_argmin} the level set method based on the adjoint approach is used.


%=======================================================================
\sectpb[Section29]{Fracture-Resistance topology optimization}
%=======================================================================

Considering the fracture effects, the topology optimization formulation of maximizing the mechanical work as an energy functional (refers to the structural toughness) is introduced as:
\begin{equation}\label{eq42}
	\begin{aligned}
		& \underset{\Phi}{\mathop{\text{Min}}}\,:\,\,\,\,J(d,\bm u,\Phi )=-\int_{\calB}\int_{\bar\varepsilon}{\bm{\sigma}(d,\bm u,\Phi )^{T}}\text{d}\bm{\varepsilon}(\bm u,\Phi)\operatorname{H}(\Phi)\text{d}{\bm{x}}, \ \\ 
		& \text{S}\text{.}\,\,\text{t}:\,\,\,\,\,\,\left\{ \begin{aligned}
			& {{\mathbf{R}}_{\text{m}}}=\nabla \cdot \bm{\sigma }(d,\bm u,\Phi)=\mathbf{0} \,\,\,\,\text{in}\,\,\calB, \ \\ 
			& {{\mathbf{R}}_{\mathbf{d}}}=[2( 1-d(\Phi))\calH(\bm u,\Phi)-d(\Phi)]+[ \ell {{s}^{2}}{{\nabla}^{2}}d(\Phi)]=\mathbf{0}\,\,\,\,\text{in}\,\,\calB,  \\ 
			& G(\Phi)=\int_{\calB}\operatorname{H}(\Phi)\text{d}{\bm{x}}=\calV(\Phi)\le \text{v}_\text{max}\text{,} \\ 
		\end{aligned} \right. \\ 
	\end{aligned}\
\end{equation}
where $ \calV(\Phi) $ and $ \text{v}_\text{max} $ are the existing volume and prescribed volume constraint, respectively. \\

Due to the nonlinear nature of the energy functional $ J $, it is approximated by the trapezoidal rule up to the prescribed displacement, depicted in Fig. \ref{Figure7}  as:
\begin{equation}
	\begin{aligned}
		J(d, \bm u,\Phi)\approx -\frac{1}{2}\sum_{\text{i=1}}^{\text{n}}{{{( {{\mathbf{F}}^{\text{i-1}}}({{d}^{\text{i}}},\Delta {{\mathbf{u}}^{\text{i}}},\Phi )\mathbf{+}{{\mathbf{F}}^{\text{i}}}({{d}^{\text{i}}},\Delta {{\mathbf{u}}^{\text{i}}},\Phi ))}^{T}}\Delta {{\mathbf{u}}^{\text{i}}}},\
	\end{aligned}\
\end{equation}
where $ \mathbf{F} $ and $ n $ are the internal force vector and number of displacement increment for finite element analysis, respectively.
\begin{figure}[!ht]
	\centering
	{\includegraphics[clip,trim=0cm 11cm 0cm 0cm, width=8cm]{Figures/P5.pdf}}  %left, bottom, right and top
	\caption{Schematic description of the trapezoidal rule estimation.
	}
	\label{Figure7}
\end{figure}


The general process of topology optimization is shown in Fig. \ref{Figure3}. As shown in Fig. \ref{Figure3}, at each iteration, the finite element method provides structural responses, and the sensitivity analysis expresses the sensitivity of the objective and constraint functions with respect to small changes in design variables. 
\begin{figure}[!ht]
	\centering
	{\includegraphics[clip,trim=1cm 5cm 2cm 2cm, width=16cm]{Figures/P3.pdf}}  %left, bottom, right and top
	\caption{Schematic description of topology optimization process.
	}
	\label{Figure3}
\end{figure}







considering a closed moving front $ S(t)=\Bx\in \R^n\ $ which is represented by zero level set of hyper surface $ \Phi (\Bx,t) $ i.e. $ S(t)=\left\{ \Bx\left| \Phi (S(t)=\Bx, t)=0\right. \right\}\ $. Taking the chain rule to calculate the time derivative of the above equation, the Hamilton-Jacobi equation is obtained as:
\begin{equation}
	\begin{aligned}
		\frac{\partial \Phi (\Bx,t)}{\partial t}=\frac{\partial \Phi (\Bx,t))}{\partial \Bx}\cdot\frac{\partial \Bx}{\partial t}=\Bv\cdot\nabla \Phi, \
	\end{aligned}
\end{equation}
\\where v is the velocity field of the closed moving front.
Since, inward normal direction is given by $ \mathbf{\vec{n}}=\frac{\nabla \Phi }{\left| \nabla \Phi  \right|}\ $the H-J equation can be replaced by:
\begin{equation}\label{eq33}
	\begin{aligned}
		\frac{\partial \Phi }{\partial t}
		=\Bv\nabla \Phi =\Bv\nabla \Phi \frac{\left| \nabla \Phi  \right|}{\left| \nabla \Phi  \right|}
		=\Bv\left| \nabla \Phi  \right|\frac{\nabla \Phi }{\left| \nabla \Phi  \right|}
		=\Bv\widehat{\Bn}\left| \nabla \Phi  \right|
		={v_{n}}\left| \nabla \Phi  \right|,
	\end{aligned}
\end{equation}
%
with $ {\mathnormal v_{n}}=\Bv.\widehat{\Bn} $ is the normal velocity field of closed moving interfaces. The \req{eq33} is the standard form for the Level Set Evolution (LSE) equation of the closed front by changing the zero level set of LSF. \TODO{@HJ--Pls give a reference.} 

%=======================================================================
\sectpb[Section30]{Reaction-Diffusion Based Level-set Method}
%=======================================================================
Since the conventional LSM with H-J evolution equation has many limitations, such as the need for initialization as the starting point that affects the final topology, the need for reshaping as a signed-distance function, the time step dependence with Courant-Friedrichs-Lewy (CFL) Conditions and inability to hole nucleation, the Reaction-Diffusion evolution is suggested as \cite{Jahan-IGA-LSM-RDE2, Jahan-IGA-LSM-RDE1, Yammada}:
\begin{equation*}
	\begin{aligned}
		\frac{\partial \Phi }{\partial t}={v_{n}}+\tau {{\nabla }^{2}}\Phi, \
	\end{aligned}
	\tag{$ \Phi$}
\end{equation*}

$\tau --> l_{\Phi}$

where $ \tau\ $is the regularization parameter. \\ Adding the diffusion term $ \tau {{\nabla }^{2}}\Phi \ $ as the Tikhonov regularization technique, provides more stabilization, smooth and well-defined boundaries \cite{Tikhonov, Yammada}.

%=======================================================================
\sectpb[Section26]{An Implicit Geometry Parameterization Based on Level Sets}
%=======================================================================
Structural boundaries, solids and holes are represented implicitly by a dynamic hypersurface as:
\begin{equation}
	\left\{	
	\begin{aligned}
		& \Phi \left( \Bx \right)>0\,\,\,\,\forall \Bx\in \Omega /\Gamma \,\,\,\,\left( \text{Solid} \right) \\ 
		& \Phi \left( \Bx \right)=0\,\,\,\,\forall \Bx\in \Gamma \bigcap \calB\,\,\left( \text{Boundary} \right) \\ 
		& \Phi \left( \Bx \right)<0\,\,\,\,\forall \Bx\in \calB/\Omega \,\,\,\,\left( \text{Void} \right), \ \\ 
	\end{aligned}
	\right.
\end{equation} 
where the zero level of the level set function is used to describe the interfaces, which represent the structural boundaries. Also, the positive and negative level set function values are used to describe solids and holes within the structure, respectively.
\begin{figure}[!t]
	\centering
	{\includegraphics[clip,trim=1cm 20cm 0cm 0cm, width=16.5cm]{Figures/intro1.pdf}}  %left, bottom, right and top
	\caption{Level set based geometric parameterization.
	}
	\label{Figure5}
\end{figure}
As shown in Fig. \ref{Figure5}, the 2-D layout is described by a 3-D LSF in which $ \calB\subset\R^d $, $ ( d=2,3 ) $ is a fixed design domain, $ \Omega\ $is a structural design configuration, including the geometry of all possible shapes, and $ \Gamma\ $represents the structural boundary that corresponds to the zero level of LSF.
%=======================================================================
\sectpb[Section27]{Geometry Projection}
%=======================================================================
An important part of the level set-based topology optimization is the geometry mapping to a structural model that affects the predicted behavior of an obtained design. The geometry mapping projects the geometry defined by the discretized LSF on the structural model that provides the structural response. The most common approach is the Eulerian approach, referred to as the density-distribution method, which leads to the evolution of materials in the fixed discretized domain. Fig. \ref{Figure6}, lists a comparison of the existing density-based approaches.\\
In the level set-based topology optimization, the Heaviside step and Dirac delta function are used to volume and boundary integration, respectively, which are defined as:
\begin{equation}
	\begin{aligned}
		\operatorname{H}\left( \Phi  \right)=\left\{ 	\begin{aligned}
			& 1,\,\,\,\,\,\,\,\,\Phi \left( \Bx \right)\ge 0 \\ 
			& 0,\,\,\,\,\,\,\,\,\Phi \left( \Bx \right)<0, \ \\ 
		\end{aligned}
		\right.
	\end{aligned}
\end{equation} 
\begin{equation}
	\begin{aligned}
		\delta (\Bx)=\frac{\partial \operatorname{H}\left( \Phi  \right)}{\partial \Bx}=\frac{\partial \operatorname{H}\left( \Phi  \right)}{\partial \Phi }\frac{\partial \Phi }{\partial \Bx}=\delta (\Phi )\left| \nabla \Phi  \right|. \ \
	\end{aligned}
\end{equation}

Therefore, considering the level set function $ \Phi (\Bx,t)\ $, the materials $ \Omega\ $and the boundaries $ \Gamma\ $of a design domain are described, respectively, as:
\begin{equation}
	\begin{aligned}
		& \Omega =\left\{ \Bx\left| \operatorname{H}(\Phi (\Bx))=1 \right. \right\}, \
	\end{aligned}
\end{equation}
\begin{equation}
	\begin{aligned}
		\Gamma =\left\{ \Bx\left| \delta (\Phi (\Bx))>0 \right. \right\}. \ 
	\end{aligned}
\end{equation}





%=======================================================================

\begin{landscape}
\begin{table}[!b] \footnotesize 
	\caption{Density-based level set methods (Eulerian Approach).}
	\centering
	\vspace{3mm}
	\label{GL-SS-eG1}
	\centering
	\begin{tabular}{  m{8em} | m{12em}| m{12em} | m{12em} | m{12em}  } 
		\hline
		& \multicolumn{2}{c|} {Direct Mapping} &  \multicolumn{2}{c}{Element-Wise Constant}  \\
		& \multicolumn{2}{c|} {(Point-Wise Density Distribution)} &  \multicolumn{2}{c}{(Material Fraction)}  \\		
		\hline		
		\multirow{2}{6em} {Description}   & Exact Heaviside Function    & Regularized Heaviside function & Material-Fraction method& Simple Direct Mapping \\ & & & Exact/Smoothed Heaviside Function & Exact/Smoothed Heaviside Function for Center of a Finite Element Cell \\		
		\hline
		\multirow{2}{6em} {Advantages} & 0/1 Manufacturable Design & Differentiable & Easy to Handle the Topological Evolution & Easy to Handle the Topological Evolution  \\ & & Easy to Handle the Topological Evolution & &  \\
		\hline		
		\multirow{8}{6em} { Disadvantages$^\star$ } & Non-Differentiable & Intermediate Densities Near the Boundaries & Non-Smooth Boundaries & Non-Smooth Boundaries  \\ 
		& Need to Represent the Interfaces Accurately & Need to Reshaping as a signed-distance function & Intermediate Density & Intermediate Density \\
		& Need to Reshaping as a signed-distance function & Need to Initialize as a Start Point & Physically Unrealistic Results & Physically Unrealistic Results  \\ 
		& Need to Initialize as a Start Point & & Convergence Problems & Convergence Problems  \\ 
		& & & Need to a Highly Refined Discretization & Need to a Highly Refined Discretization  \\ 
		& & & Non-Differentiable if Using the Exact Heaviside Function & Non-Differentiable if Using the Exact Heaviside Function \\ 
		& & & Need to Reshaping as a signed-distance function & Need to Reshaping as a signed-distance function  \\ 
		& & & Need to Initialize as a Start Point & Need to Initialize as a Start Point  \\
		\hline		
	\end{tabular}\\[1.8mm]
	{\parbox{10in}{{${\star} ~$\textit{When the RDE is used, the shape and topology evolve accurately without the need to reshaping and initialization.}}}}
\end{table}
\end{landscape}


%=======================================================================
\sectpb[Section29]{Sensitivity Analysis}
%=======================================================================

%=======================================================================
\sectpb[Section29]{Space-time finite element discretization}
%=======================================================================

In this section, we provide discretizations of the variational forms given in Algorithm \ref{SDTableGL-DN}. These equations stem from the Global-Local formulation augmented with Dirichlet-Neumann-type boundary conditions, i.e., $g/l-1$. Thus, the space-discrete variational formulation via finite element approximation for the local and global BVPs are discussed.
	
Let $\mathcal{P}$ be a finite element partition of $\calB$ into quadrilaterals, and $N_i$ denotes the nodal shape function associated with the node $i$. The scalar-valued quantity $\hat{\bullet}_i$ represents the nodal value. For the global-local formulation, we assume the existence of the partitions $\mathcal{P}_G$ and $\mathcal{P}_L$. The solution discretization are given by
\begin{equation}
	\Bu^h=\BN_\Bu\hat{\bm u}, \quad
	d^h=\bm{N}_d\hat{\bm d}, \quad
	\Phi^h=\bm N_u\hat{\Phi}.
	\label{Discr1}
\end{equation}
and its derivative
\begin{equation}
	\bm\varepsilon(\bm u_h)=\bm B_u\hat{\bm u}, \quad
	\nabla d_h=\bm B_d\hat{\bm d}, \quad
	\nabla \Phi_h=\bm B_d\hat{\Phi}.
	\label{Discr2}
\end{equation}

%
\begin{equation}
    {{\bf{R}}_\Bu}=
    \sum_{e} \int_{\calB_e}\big[{\BB^T_\Bu} \Bsigma_h(\Bve,\Bve^p,d;\Phi)-\overline{\Bf}\cdot\BN_\Bu\big]\,dv - \int_{\partial\calB_N}\overline{\Btau}\cdot\BN_\Bu\,da ={\bm 0}, 
	\label{phf_fem_u}
\end{equation}
%

%
\begin{equation}
{{\bf{R}}_d}=
\sum_{e}\int_{\calB_e} \bigg[ \bigg((1-d^h)\calH_h -  {d} + \frac{\eta_d}{\Delta t}(d^h-d^h_n)\bigg)\cdot\BN_d- l_d^2  \BB_d^T\cdot\nabla d_h \bigg]\,dv ={\bm 0}. 
	\label{phf_fem_d}
\end{equation}
%

%
\begin{equation}
	{{\bf{R}}_\Phi}=
	\sum_{e}\int_{\calB_e} \bigg[ \bigg( v_h - \frac{1}{\Delta t}(\Phi^h-\Phi^h_n)\bigg)\cdot\BN_d- l_\Phi^2  \BB_\Phi^T\cdot\nabla \Phi_h \bigg]\,dv ={\bm 0}. 
	\label{phf_fem_phi}
\end{equation}
%

Here, $\square$ is related to $\bm{\lambda},\Bu$ and $\bullet$ indicates $G, L$. Accordingly, its constitutive state variables are represented by $(\Bve^{h}_{G}, \Bve^{h}_{L}, \BG_{L}^{h})$
%

Here, $\BB_{\Bu}^{G,i}$, $\BB_{\Bu}^{L,i}$, and $\BB_{s}^{L,i}$ are the matrix representation for the $i^{th}$ nodal shape function's derivative, corresponding to the global deformation, local deformation and local crack phase-field, respectively. 



Discretization of the local BVP is aimed at determining the primary fields
$({\Bu}_L,s_L,\bm\lambda_L)$ via finite element approximation. To do so, for each primary field, the set of discretized equilibrium equations based on the \textit{residual} force vector denoted by $\BR^{\bullet}$ has to be determined. Thus, for the crack phase-field part we have,
\begin{equation}\label{SDfemND1}
	\begin{aligned}
		{{\bf{R}}^s_L}= 
		\bigcup_{e=1} \sum_{i} \Big(
		\int_{\calB_e} \big({{N_s^{L,i}}\big)^{T}\Big[ {g^{\prime}(s^{h}_+)\calH(\bm\varepsilon(\bm u^{h}_L))}+(s^{h}_{L}-1)\Big] \ \mathrm{d}{\Bx}}\\
		+\int_{\calB_e} \big({{\bm B_s^{L,i}}\big)^{T} {l^2 \nabla s^{h}_L} \ \mathrm{d}{\Bx}}\Big)={\bm 0}, 
	\end{aligned}
\end{equation}
with
\begin{equation*}\label{SDfemND10}
	g^{\prime}(s^{h}_+)=2(1-\kappa)s^{h}_{L+},
\end{equation*}

and for the local mechanical part, we have
\begin{equation}\label{SDfemND2}
	\begin{aligned}
		\begin{cases}
			{{\bf{R}}^{\Bu}_L}= \bigcup_{e=1} \sum_{i} \int_{\calB_e} \Big({{\bm B_\Bu^{L,i}}\Big)^{T} {{\bm\sigma}_h(\bm u_L,s_L)} \ \mathrm{d}{\Bx}}
			-{\bf{J}}_L^{T}\hat{\bm\lambda}_L{=}{\bm 0}, \\\\
			{{\bf{R}}^{ {\text{C}}_3}_L}= {\bf{L}}_L{\hat{\Bu}^{k-1}_{\Gamma}-{\bf{J}}_L{\hat{\Bu}_L}}{=}{\bm 0},
		\end{cases}
	\end{aligned}
\end{equation}


	\cleardoublepage
+++++++++++++++++++
in order to derive the gradient-based fully coupled adjoint-based sensitivity analysis, derivatives of the objective and constraint functions with respect to the design variables need to be provided to evolve the structural topology. Considering $ \bm{\eta }\ $and $ \bm{\gamma }\ $as the adjoint vectors, the Lagrangian function of the optimization problem can be expressed as:
\begin{equation}\label{LGforopt}
	\begin{aligned}
	\BfrakL(\Phi,{\bm\lambda_{\Bu}},{\bm\lambda_{d}},{\lambda_{V}};\bar{\Bu},\bar{d},\bar{\alpha})
	=\sum_{\text{i}=1}^{n}\Big({J}^{\text{i}}
	+({\bm\mu^{i}_{\Bu}})^T\mathbf{R}^{i-1}_\Bu
	+({\bm\lambda^{i}_{\Bu}})^T\mathbf{R}^{i}_\Bu
	+({\bm\lambda^{i}_{d}})^T \mathbf{R}^{i}_\text{d}\Big)
	+ {\lambda^{T}_{V}} \text{G}(\Phi) . \ \\
	\end{aligned}\	
\end{equation}
%
with
%
\begin{equation}
	J=\sum_{\text{i}=1}^{n} {J^i} \WITH J^i=-\frac{1}{2}(\BR^{i}_\Bu+\BR^{i-1}_\Bu).(\Bu^i-\Bu^{i-1})
\end{equation}
%


%
\begin{equation}\label{compat_argmin2}
	\fterm{ 
		\{ \Phi,{\bm\lambda_{\Bu}},{\bm\lambda_{d}},{\bm\lambda_{V}}\} = 
		\mbox{arg} \{\; 
		\substackrel{\bm{u} \in \bf{V} }{\mbox{min}}
		\substackrel{d \in W_{in} }{\mbox{min}} \,
		[\; \BfrakL(\bm u,d,\Phi) \; ]
		\; \}.
	}
\end{equation}
%

%,{\bm\lambda_{\Bu}},{\bm\lambda_{d}}
	
To perform the adjoint sensitivity, the derivatives of the Lagrangian function with respect to the design variables can be expressed as:




%
\begin{equation}\label{eq45}
	\begin{aligned}
		\mathcal{G}(\Phi;\Bu,d)
		:=D_{\Phi} \BfrakL
		&=\sum_{\text{i}=1}^{n} \Big(
		D_{\Phi} J^i
		+({\bm\mu^{i}_{\Bu}})^TD_{\Phi} \BR_\Bu^{i-1}
		+({\bm\lambda^{i}_{\Bu}})^TD_{\Phi} \BR_\Bu^{i}\\[2 mm]
		&+({\bm\mu^{i-1}_{d}})^TD_{\Phi} \BR_d^{i-1}
		+({\bm\lambda^{i}_{d}})^TD_{\Phi} \BR_d^{i}
		\Big)\\[2 mm]
		&+{\lambda^{T}_{V}} \frac{d \text{G}(\Phi)}{d \Phi}
	\end{aligned}\
\end{equation}
%


%
\begin{equation}\label{eq:sens_J}
	\begin{aligned}
		D_{\Phi} J^i=
	    -\frac{1}{2}\Big(   D_{\Phi} \BR_\Bu^{i-1} +D_{\Phi} \BR_\Bu^{i} \Big)\Delta \Bu^i
	    -\frac{1}{2}\Big( \BR_\Bu^{i-1}+\BR_\Bu^{i}\Big) \frac{d \Delta \Bu^i}{d\Phi} 
	\end{aligned}\
\end{equation}
%

%\begin{equation}\label{eq:sens_R_u}
%	\begin{aligned}
%		D_{\Phi} \BR_\Bu^{\bullet}
%		&=\frac{d \BR_\Bu^{\bullet}}{d \Phi}
%		+\frac{\partial \BR_\Bu^{\bullet}}{d \Delta \Bu^{\bullet}}\cdot\frac{d\Delta \Bu^{\bullet}}{d\Phi}
%		+\frac{\partial \BR_\Bu^{\bullet}}{d  d^{\bullet}}\cdot\frac{dd^{\bullet}}{d\Phi}\\[2 mm]
%		&=\frac{d \BR_\Bu^{\bullet}}{d \Phi}
%		+\BK_{\Bu,\Bu}^{\bullet} \cdot\frac{d\Delta \Bu^{\bullet}}{d\Phi}
%		+\BK_{\Bu,d}^{\bullet} \cdot\frac{d d^{\bullet}}{d\Phi}
%		\quad \text{for} \quad \bullet=\{i-1,i\}%\\[2 mm]
%	\end{aligned}\
%\end{equation}

\begin{equation}\label{eq:sens_R_u_i_1}
	\begin{aligned}
		D_{\Phi} \BR_\Bu^{i-1}
		&=\frac{d \BR_\Bu^{i-1}}{d \Phi}
		+\frac{\partial \BR_\Bu^{i-1}}{d \Delta \Bu^{i-1}}\cdot\frac{d\Delta \Bu^{i-1}}{d\Phi}
		+\frac{\partial \BR_\Bu^{i-1}}{d  d^{i-1}}\cdot\frac{dd^{i-1}}{d\Phi}\\[2 mm]
		&=\frac{d \BR_\Bu^{i-1}}{d \Phi}
		+\BK_{\Bu,\Bu}^{i-1} \cdot\frac{d\Delta \Bu^{i-1}}{d\Phi}
		+\BK_{\Bu,d}^{i-1} \cdot\frac{d d^{i-1}}{d\Phi}
	\end{aligned}
	\end{equation}

\begin{equation}\label{eq:sens_R_u_i}
	\begin{aligned}
		D_{\Phi} \BR_\Bu^{i}
		&=\frac{d \BR_\Bu^{i}}{d \Phi}
		+\frac{\partial \BR_\Bu^{i}}{d \Delta \Bu^{i}}\cdot\frac{d\Delta \Bu^{i}}{d\Phi}
		+\frac{\partial \BR_\Bu^{i}}{d  d^{i}}\cdot\frac{dd^{i}}{d\Phi}\\[2 mm]
		&=\frac{d \BR_\Bu^{i}}{d \Phi}
		+\BK_{\Bu,\Bu}^{i} \cdot\frac{d\Delta \Bu^{i}}{d\Phi}
		+\BK_{\Bu,d}^{i} \cdot\frac{d d^{i}}{d\Phi}
	\end{aligned}
\end{equation}


\begin{equation}\label{eq:sens_R_d_i_1}
	\begin{aligned}
		D_{\Phi} \BR_d^{i-1}
		&=\frac{d \BR_d^{i-1}}{d \Phi}
		+\frac{\partial \BR_d^{i-1}}{d \Delta \Bu^{i-1}}\cdot\frac{d\Delta \Bu^{i-1}}{d\Phi}
		+\frac{\partial \BR_d^{i-1}}{d  d^{i-1}}\cdot\frac{dd^{i-1}}{d\Phi}\\[2 mm]
		&=\frac{d \BR_d^{i-1}}{d \Phi}
		+\BK_{d,\Bu}^{i-1} \cdot\frac{d\Delta \Bu^{i-1}}{d\Phi}
		+\BK_{d,d}^{i-1} \cdot\frac{d d^{i-1}}{d\Phi}%
	\end{aligned}\
\end{equation}


\begin{equation}\label{eq:sens_R_d_i}
	\begin{aligned}
		D_{\Phi} \BR_d^{i}
		&=\frac{d \BR_d^{i}}{d \Phi}
		+\frac{\partial \BR_d^{i}}{d \Delta \Bu^{i}}\cdot\frac{d\Delta \Bu^{i}}{d\Phi}
		+\frac{\partial \BR_d^{i}}{d  d^i}\cdot\frac{dd^{i}}{d\Phi}\\[2 mm]
		&=\frac{d \BR_d^{i}}{d \Phi}
		+\BK_{d,\Bu}^{i} \cdot\frac{d\Delta \Bu^{i}}{d\Phi}
		+\BK_{d,d}^{i} \cdot\frac{d d^{i}}{d\Phi}%
	\end{aligned}\
\end{equation}



\begin{equation}
	\begin{aligned}	
		\frac{d }{d \Phi }\text{G}(\Phi)=\int_{\calB}{\delta \left( \Phi \right)\mathrm{d}{\bm{x}} }. 
	\end{aligned}\
\end{equation}


%
\begin{equation}\label{eq45}
	\begin{aligned}
		\mathcal{G}(\Phi;\Bu,d)=
		&({\bm\mu^{i}_{\Bu}}-\frac{1}{2}\Delta \Bu^{i})^T\frac{d \BR_\Bu^{i-1}}{d \Phi}
		+({\bm\lambda^{i}_{\Bu}}-\frac{1}{2}\Delta \Bu^{i})^T\frac{d \BR_\Bu^{i}}{d \Phi}\\[2 mm]
		&+({\bm\mu^{i}_{d}}-\frac{1}{2}\Delta d^{i})^T\frac{d \BR_d^{i-1}}{d \Phi}
		+({\bm\lambda^{i}_{d}}-\frac{1}{2}\Delta d^{i})^T\frac{d \BR_d^{i}}{d \Phi}\\[2 mm]
		&+\Big(
		({\bm\mu^{i}_{\Bu}}-\frac{1}{2}\Delta \Bu^{i})^T \BK_{\Bu,\Bu}^{i-1}
		+({\bm\mu^{i}_{d}}-\frac{1}{2}\Delta d^{i})^T \BK_{d,\Bu}^{i-1}
		\Big)\cdot \frac{d\Delta \Bu^{i-1}}{d\Phi}\\[2 mm]
		&+\Big(
		({\bm\lambda^{i}_{\Bu}}-\frac{1}{2}\Delta \Bu^{i})^T \BK_{\Bu,\Bu}^{i}
		+({\bm\lambda^{i}_{d}}-\frac{1}{2}\Delta d^{i})^T \BK_{d,\Bu}^{i}
		\Big)\cdot \frac{d\Delta \Bu^{i}}{d\Phi}\\[2 mm]
		&+\Big(
		({\bm\mu^{i}_{\Bu}}-\frac{1}{2}\Delta \Bu^{i})^T \BK_{\Bu,d}^{i-1}
		+({\bm\mu^{i}_{d}}-\frac{1}{2}\Delta d^{i})^T \BK_{d,d}^{i-1}
		\Big)\cdot \frac{d\Delta d^{i-1}}{d\Phi}\\[2 mm]
		&+\Big(
		({\bm\lambda^{i}_{\Bu}}-\frac{1}{2}\Delta \Bu^{i})^T \BK_{\Bu,d}^{i}
		+({\bm\lambda^{i}_{d}}-\frac{1}{2}\Delta d^{i})^T \BK_{d,d}^{i}
		\Big)\cdot \frac{d\Delta d^{i}}{d\Phi}\\[2 mm]
		&-\frac{1}{2}\Big( \BR_\Bu^{i-1}+\BR_\Bu^{i}\Big) \frac{d \Delta \Bu^i}{d\Phi} \\[2 mm]
		&-\frac{1}{2}\Big( \BR_d^{i-1}+\BR_d^{i}\Big) \frac{d \Delta d^i}{d\Phi} 
	\end{aligned}\
\end{equation}
%


Using chain rule, the sensitivity of each term of the \req{eq45} can be written as:


\begin{equation}
	123
\end{equation}




\begin{equation} 
	\begin{aligned}
		\frac{\partial }{\partial \Phi }J=-\frac{1}{2}{{\left( \frac{\mathrm{d}}{\mathrm{d}\Phi}\left( {{\mathbf{F}}^{\text{i-1}}}\mathbf{+}{{\mathbf{F}}^{\text{i}}} \right) \right)}^{T}}\Delta {{\mathbf{u}}^{\text{i}}}-\frac{1}{2}\left( {{\left( \frac{\partial }{\partial \Delta {{\mathbf{u}}^{\text{i}}}}\left( {{\mathbf{F}}^{\text{i-1}}}\mathbf{+}{{\mathbf{F}}^{\text{i}}} \right) \right)}^{T}}\Delta {{\mathbf{u}}^{\text{i}}} \right)\frac{\partial \Delta {{\mathbf{u}}^{\text{i}}}}{\partial \Phi }-\\ \frac{1}{2}{{\left( {{\mathbf{F}}^{\text{i-1}}}\mathbf{+}{{\mathbf{F}}^{\text{i}}} \right)}^{T}}\frac{\partial \Delta {{\mathbf{u}}^{\text{i}}}}{\partial\Phi}-\frac{1}{2}\left( \frac{\partial }{\partial {{d}^{\text{i}}}}{{\left( {{\mathbf{F}}^{\text{i-1}}}\mathbf{+}{{\mathbf{F}}^{\text{i}}} \right)}^{T}}\Delta {{\mathbf{u}}^{\text{i}}} \right)\frac{\partial {{d}^{\text{i}}}}{\partial\Phi}, 
	\end{aligned}\
\end{equation}
\begin{equation}
	\begin{aligned}
		\frac{\partial }{\partial\Phi}\left( \mathbf{R}_{\text{m}}^{\text{i-1}}+\mathbf{R}_{\text{m}}^{\text{i}} \right)=\frac{\mathrm{d}}{\mathrm{d}\Phi}\left( \mathbf{R}_{\text{m}}^{\text{i-1}}+\mathbf{R}_{\text{m}}^{\text{i}} \right)+\frac{\partial }{\partial \Delta {{\mathbf{u}}^{\text{i}}}}\left( \mathbf{R}_{\text{m}}^{\text{i-1}}+\mathbf{R}_{\text{m}}^{\text{i}} \right)\frac{\partial \Delta {{\mathbf{u}}^{\text{i}}}}{\partial \Phi}+\\  \frac{\partial }{\partial {{d}^{\text{i}}}}\left( \mathbf{R}_{\text{m}}^{\text{i-1}}+\mathbf{R}_{\text{m}}^{\text{i}} \right)\frac{\partial {{d}^{\text{i}}}}{\partial\Phi}, 
	\end{aligned}\
\end{equation}
\begin{equation}
	\begin{aligned}
		\frac{\partial }{\partial\Phi}\mathbf{R}_{\text{d}}^{\text{i}}=\frac{\mathrm{d}}{\mathrm{d}\Phi}\mathbf{R}_{\text{d}}^{\text{i}}+\frac{\partial }{\partial \Delta {{\mathbf{u}}^{\text{i}}}}\mathbf{R}_{\text{d}}^{\text{i}}\frac{\partial \Delta {{\mathbf{u}}^{\text{i}}}}{\partial\Phi}+\frac{\partial }{\partial {{d}^{\text{i}}}}\mathbf{R}_{\text{d}}^{\text{i}}\frac{\partial {{d}^{\text{i}}}}{\partial\Phi }, 
	\end{aligned}\
\end{equation} 
\begin{equation}
	\begin{aligned}	
		\frac{\partial }{\partial \Phi }G=\int_{\calB}{\delta \left( \Phi \right)\mathrm{d}{\bm{x}} }. 
	\end{aligned}\
\end{equation}

To eliminate the implicit derivatives, the terms containing $ \frac{\partial \Delta {{\mathbf{u}}^{\text{i}}}}{\partial \Phi }\ $and $ \frac{\partial {{d}^{\text{i}}}}{\partial \Phi}\ $must be equal to zero. This leads to solving the following expressions for the adjoint vectors $ \bm{\eta }\ $and $ \bm{\gamma }\ $ based on the staggered method until the residuals of $ \left( {{\bm{\eta }}^{i}}-{{\bm{\eta }}^{i-1}} \right)\ $and $ \left( {{\bm{\gamma }}^{i}}-{{\bm{\gamma }}^{i-1}} \right)\ $reaches less than a predefined small value.

To eliminate the implicit derivatives, the terms between square b rackets must be equal to zero.

\begin{equation}
	\begin{aligned}	
		& \left( -\frac{1}{2}\left( {{\left( \frac{\partial }{\partial \Delta {{\mathbf{u}}^{\text{i}}}}\left( {{\mathbf{F}}^{\text{i-1}}}\mathbf{+}{{\mathbf{F}}^{\text{i}}} \right) \right)}^{T}}\Delta {{\mathbf{u}}^{\text{i}}} \right)-\frac{1}{2}{{\left( {{\mathbf{F}}^{\text{i-1}}}\mathbf{+}{{\mathbf{F}}^{\text{i}}} \right)}^{T}}+\frac{\partial }{\partial \Delta {{\mathbf{u}}^{\text{i}}}}{{\left( \mathbf{R}_{\text{m}}^{\text{i-1}}+\mathbf{R}_{\text{m}}^{\text{i}} \right)}^{T}}\bm{\eta }+\frac{\partial }{\partial \Delta {{\mathbf{u}}^{\text{i}}}}\mathbf{R}_{\text{d}}^{{{\text{i}}^{T}}}\bm{\gamma } \right)\frac{\partial \Delta {{\mathbf{u}}^{\text{i}}}}{\partial \Phi }=\mathbf{0},  \\ 
		& \left( -\frac{1}{2}\left( \frac{\partial }{\partial {{d}^{\text{i}}}}{{\left( {{\mathbf{F}}^{\text{i-1}}}\mathbf{+}{{\mathbf{F}}^{\text{i}}} \right)}^{T}}\Delta {{\mathbf{u}}^{\text{i}}} \right)+\frac{\partial }{\partial {{d}^{\text{i}}}}\left( \mathbf{R}_{\text{m}}^{\text{i-1}}+\mathbf{R}_{\text{m}}^{\text{i}} \right)\bm{\eta }+\frac{\partial }{\partial {{d}^{\text{i}}}}\mathbf{R}_{\text{d}}^{{{\text{i}}^{T}}}\bm{\gamma } \right)\frac{\partial {{d}^{\text{i}}}}{\partial \Phi }=\mathbf{0}. \\ 
	\end{aligned}\
\end{equation}

Substituting the obtained adjoint variables into \req{eq45} yields the sensitivity of the Lagrangian function as:
\begin{equation}\label{eq51}
	\begin{aligned}
		\mathcal{G}=\underbrace{\sum\limits_{\text{i}=1}^{n}{\left( -\frac{1}{2}{{\left( \frac{\mathrm{d}}{\mathrm{d}\Phi}\left( {{\mathbf{F}}^{\text{i-1}}}\mathbf{+}{{\mathbf{F}}^{\text{i}}} \right) \right)}^{T}}\Delta {{\mathbf{u}}^{\text{i}}}+\frac{\mathrm{d}}{\mathrm{d}\Phi}{{\left( \mathbf{R}_{\text{m}}^{\text{i-1}}+\mathbf{R}_{\text{m}}^{\text{i}} \right)}^{T}}{{\bm{\eta }}^{\text{i}}}+\frac{\mathrm{d}}{\mathrm{d}\Phi}\mathbf{R}_{\text{d}}^{{{\text{i}}^{T}}}{{\bm{\gamma }}^{\text{i}}} \right)}}_{\mathcal{G}_S}
		+\underbrace{\lambda \int_{\calB}{\delta \left( \Phi \right)\mathrm{d}{\bm{x}} }}_{\mathcal{G}_V}. \\
	\end{aligned}\	
\end{equation}
%
so,
%
\begin{equation}
	\mathcal{G}=\mathcal{G}_S+\mathcal{G}_V
\end{equation}
%
which is now modified to
%
\begin{equation}
	\mathcal{G}=\widehat{\mathcal{G}}_S+\mathcal{G}_V
\end{equation}
%
The level set velocity field required for closed front propagation is obtained from the steepest descent method. For this reason, the derivative of the Lagrangian function with respect to pseudo time gives:
\begin{equation}
	\begin{aligned}
		\frac{\partial \mathcal{L}}{\partial t}=\frac{\partial \mathcal{L}}{\partial \Phi }.\frac{\partial \Phi }{\partial \Bx}.\frac{\partial \Bx}{\partial t}=\mathcal{G}{\bm{\text{v}}_{n}}\left| \nabla \Phi  \right|. \\
	\end{aligned}
\end{equation}

Substituting the obtained time derivative into integration form of \req{eq51} yields:
\begin{equation}
	\begin{aligned}
		\frac{\partial \mathcal{L}}{\partial t}=\int_{\calB}{\mathcal{G}\delta \left( \Phi  \right){\bm{\text{v}}_{n}}\left| \nabla \Phi  \right|\mathrm{d}{\bm{x}} }=\int_{\partial\calB}{\mathcal{G}{\bm{\text{v}}_{n}}\mathrm{d}{\bm{s}}}. \\
	\end{aligned}
\end{equation}

Therefore, the normal velocity field of the optimization formulation \req{eq42}, is defined as:
\begin{equation}
	\begin{aligned}
		{\bm{\text{v}}_{n}}\left| _{\Phi = 0} \right.=-\mathcal{G}. \
	\end{aligned}
\end{equation}

By extracting the normal velocity field of the optimization problem, the \req{eq33} will be able to provide the optimal topology for PDE based LSM. For variational based LSM, LSE equation is given by $ \frac{\partial \Phi }{\partial t}={\bm{\text{v}}_{n}}\text{ }\!\!\delta\!\!\text{ }\left( \Phi  \right)\ $.

\begin{Remark}
	\label{rem:augumentedLG}
	We note that in this work, Legrangian method is used, while one can simply extend the method toward augumented Legrangian method. To do so, modified Lagrange variable introduced as ${\widehat{\bm\lambda}^{T}_{\Bu}}={\bm\lambda^{T}_{\Bu}}+\frac{p_u}{2}(\mathbf{R}^{i-1}_\Bu
	+\mathbf{R}^{i}_\Bu)$ for mechanical part, ${\widehat{\bm\lambda}^{T}_{d}}={\bm\lambda^{T}_{d}}+\frac{p_d}{2}( \mathbf{R}^{i}_\text{d})$ for phase-field part, and ${\widehat{\lambda}^{T}_{V}}={\lambda^{T}_{V}}+\frac{p_V}{2}( G(V))$. So, \req{LGforopt} will be changed toward $\BfrakL(\Phi,{\widehat{\bm\lambda}_{\Bu}},{\widehat{\bm\lambda}_{d}},{\widehat{\lambda}_{V}};\bar{\Bu},\bar{d},\bar{\alpha})$ for set of unknowns $(\Phi,{\bm\lambda_{\Bu}},{\bm\lambda_{d}},{\lambda_{V}})$.
\end{Remark}


%=======================================================================
\sectpb[Section31]{Lagrange Multiplier}
%=======================================================================
A gradually convergence Bi-Sectioning algorithm is used to satisfy the volume constraint which has been initialized using a lower $ {{\lambda }_{l}} $ and an upper $ {{\lambda }_{b}} $ bound for the Lagrange multiplier \cite{Sigmond1}. 
to update the interval of the Lagrange multiplier, the following scheme has been used:
\begin{equation}\label{eq56}
	\begin{aligned}
		\lambda =\sqrt{{{\lambda }_{l}}{{\lambda }_{b}}}. \\
	\end{aligned}
\end{equation}

Then, if the available volume is more than the expected volume, ${{\lambda }_{l}}$ will be replaced by $ \lambda\ $ and if it is less than the expected volume, ${{\lambda }_{b}}$ will be replaced by $ \lambda \ $.
Also, in order to gradually reduce the material, the expected volume is updated iteratively as:
\begin{equation}\label{eq57}
	\begin{aligned}
		{{\text{v}}^{*}}=\text{v}\left( \Phi  \right)-0.01\left( \calV\left( \Phi  \right)-{{\text{v}}_{\max }} \right). \\
	\end{aligned}
\end{equation}
\begin{algorithm}[H]\small
	\caption{\em Bi-section procedure.}
	\label{alg_1}
	Let $\texttt{TOL} $ be a given. find corresponding $ \lambda\in\R^+\ $which must be modified using the following steps:
	\begin{enumerate}
		\item Choose lower ${{\lambda }_{l}}$ and upper ${{\lambda }_{b}}$ guesses such that the volume constraint function changes sign over the interval, \\ [2 mm]
		\item Find the new estimate of the $\lambda\ $ from \req{eq56},	
		\item Construct the criterion such as ($  |G| < \texttt{TOL} $), 
		\item{\it Checking criterion with the limitation obtained from \req{eq57}:} If "\texttt{No}" proceed {to step 2.}
		If "\texttt{Yes}" break,
		\item If $ \texttt{G} > \texttt{+TOL} $ then ${{\lambda }_{l}}= \lambda\ $ and proceed to step 2,
		\item If $ \texttt{G} < \texttt{-TOL} $ then ${{\lambda }_{b}}= \lambda\ $ and proceed to step 2,
	\end{enumerate}
\end{algorithm}
%=======================================================================
\sectpb[Section31]{Numerical Implementation}
%=======================================================================
Since the point-wise exact Heaviside step function is employed for geometry mapping, when a hole is nucleated in an appropriate region, its sensitivity is always zero and no material can be added to that domain which is the so-called evolution locking. So, a sensitivity filter scheme has been used to provide the potential for material creation in the void regions. To the best of the authors' knowledge, the filter schemes are used to overcome the numerical instabilities of topology optimization such as intermediate densities, mesh dependency, checkerboard patterns and local minima that occur in element-wise constant density distribution techniques such as SIMP and ESO \cite{diaz, sigmond2, sigmund4, sigmund3}.
The formulation of symmetric sensitivity filter without density weighting scheme is written as \cite{Sigmund5}:
\begin{equation}
	\begin{aligned}
		{\mathcal{\widetilde{G}}_{S,i}}=\frac{\sum\limits_{j\in {{N}_{n}}}{w\left( {\Bx_{ij}} \right){\mathcal{G}_{S,j}}}}{\sum\limits_{j\in {{N}_{n}}}{w\left( {\Bx_{ij}} \right)}}, \\
	\end{aligned}
\end{equation}
where $ {{N}_{n}}\ $ and $ w\left( {\Bx_{ij}} \right)\ $ denotes the number of nodes and weight factor, respectively.
The smooth continuous weight factor is defined as:
\begin{equation}\label{eq59}
	\begin{aligned}
		w\left( {\Bx_{ij}} \right)={{e}^{-3{{(\frac{\left\| {\Bx_{ij}}-{\Bx_{ni}} \right\|}{{{R}_{\min }}})}^{3}}}}, \\
	\end{aligned}
\end{equation}
where $ {\Bx_{ni}}\ $and $ {{R}_{\min }}\ $ denotes the spatial coordinates of i-th node and filter radius, respectively. Fig. 8 illustrates the nonlinear filter factor in a 2D mesh using \req{eq59}, schematically.
\begin{figure}[!ht]
	\centering
	{\includegraphics[clip,trim=0cm 8cm 0cm 8cm, width=10cm]{Figures/P7.pdf}}  %left, bottom, right and top
	\caption{Schematic description of the weight function used in sensitivity filtering.
	}
	\label{Figure8}
\end{figure}				
The result obtained from the sensitivity filter is still a chaotic phenomenon and the optimization process may fail to converge. to overcome this obstacle, sensitivities are averaged with their historical information, which is written as:
\begin{equation}
	\begin{aligned}
		\widehat{\mathcal{G}}_{S,i}=\frac{\widetilde{\mathcal{G}}_{S,i}+\widehat{\mathcal{G}}_{S,i}^{k-1}+\widehat{\mathcal{G}}_{S,i}^{k-2}}{3}\,\,\,\,\,with\,\,\,\,k>2.\
	\end{aligned}
\end{equation}

NOTE $k$ is the iteration of optimization.
So, $ \overset\frown{\mathcal{G}}_{S,i}^{k}\ $ is employed as the normal velocity field to update the design variable and evolution of the LSF.

%\begin{figure}[!ht]
%	\centering
%	{\includegraphics[clip,trim=0cm 17cm 0cm 0cm, width=18cm]{Figures/T1.pdf}}  %left, bottom, right and top
%	\caption{Schematic description of the weight function used in sensitivity filtering.
%	}
%	\label{Figure8}
%\end{figure}












